Language GANs Falling Short

Generating high-quality text with sufficient diversity is essential for a wide range of Natural Language Generation (NLG) tasks. Maximum-Likelihood (MLE) models trained with teacher forcing have consistently been reported as weak baselines, where poor performance is attributed to exposure bias (Bengio et al., 2015; Ranzato et al., 2015); at inference time, the model is fed its own prediction instead of a ground-truth token, which can lead to accumulating errors and poor samples. This line of reasoning has led to an outbreak of adversarial based approaches for NLG, on the account that GANs do not suffer from exposure bias. In this work, we make several surprising observations which contradict common beliefs. First, we revisit the canonical evaluation framework for NLG, and point out fundamental flaws with quality-only evaluation: we show that one can outperform such metrics using a simple, well-known temperature parameter to artificially reduce the entropy of the model's conditional distributions. Second, we leverage the control over the quality / diversity trade-off given by this parameter to evaluate models over the whole quality-diversity spectrum and find MLE models constantly outperform the proposed GAN variants over the whole quality-diversity space. Our results have several implications: 1) The impact of exposure bias on sample quality is less severe than previously thought, 2) temperature tuning provides a better quality / diversity trade-off than adversarial training while being easier to train, easier to cross-validate, and less computationally expensive. Code to reproduce the experiments is available at github.com/pclucas14/GansFallingShort

==> old.tex <==
% Introduction
% Liam:  This paragraph is simply too generic and not relevant to this work.  It seeks to motivate why someone would care about GANs
% but this is not our objective of this paper.  Truncate.
Through architecture advances, improved training techniques, and larger datasets, the natural language processing (NLP) community has developed generative models achieving ever lower (held-out) perplexities, and increasingly more compelling samples.
Building off improved models like the transformer \citep{vaswani2017attention}, recent work has pushed models with parameter counts numbering in the billions, and consuming larger datasets, to yield impressive results \citep{radford2018improving, devlin2018bert, radford2019language}.
However, virtually all learning still relies on MLE-training and sequential decomposition of the joint distribution, which is potentially subject to \emph{exposure bias} \citep{bengio2015scheduled,ranzato2015sequence}.
The ground truth sequence is fed in during training, and the model aims to maximize the likelihood of conditional distributions.
However, for generation, the model samples autoregressively from its previously generated tokens to produce samples.
Generally, models that achieve lower perplexity have been shown to produce better samples in the conditional generation domain \citep{radford2019language}, but it is not an explicit objective of the training procedure.

Therefore, motivated by the success of GANs in image generation \citep{goodfellow2014generative, radford2015unsupervised}, by the perception that exposure bias significantly degrades the performance of MLE trained models, and by a training procedure that explicitly aims to improve sample quality (to a learned critic) numerous GAN-models for text generation have been proposed


Assessing \emph{sample generation} via adequate and robust evaluation metrics remains a challenge for image generation \citep{theis2015note,barratt2018note}. 
Rather than held-out likelihood, model performance is often assessed by evaluating generated samples. In this case, the gold standard is to perform human evaluation. This is however impractical and expensive.

% % Quality-diversity
% % Models should generate high-quality and highly-diverse samples. 
% Using two different evaluation measures can make it difficult to compare models.
% This is exemplified in Figure \ref{fig:new_eval} (left).
% The performance of two models is plotted, and each one does better in one of the two dimensions.
% Without further information about the trade-off between the two dimensions, it is impossible to state which is superior.

